Learning to simulate partially known spatio-temporal dynamics with trainable difference operators

Recently, using neural networks to simulate spatio-temporal dynamics has received a lot of attention. However, most existing methods adopt pure data-driven black-box models, which have limited accuracy and interpretability. By combining trainable difference operators with black-box models, we propose a new hybrid architecture explicitly embedded with partial prior knowledge of the underlying PDEs named PDE-Net++. Furthermore, we introduce two distinct options called the trainable flipping difference layer (TFDL) and the trainable dynamic difference layer (TDDL) for the difference operators. Numerous numerical experiments have demonstrated that PDE-Net++ has superior prediction accuracy and better extrapolation performance than black-box models.

==> sections/TDDL_alg.tex <==

\begin{algorithm}
    \caption{Trainable Dynamic Difference Layer (TDDL)}\label{alg:TDDL}
    \begin{algorithmic}[1]
        \STATE \textbf{initialize} $K_{uv}^0$ for all possible $u$ and $v$ by Prop. \ref{prop:kernels-in-hyperplane} with $L$, $\Delta x$, $\Delta y$ defined in Sec. \ref{sec:tddl}

        \item[]
        \FUNCTION{TDDL($h$, \texttt{pqr\_list})}%\COMMENT{\texttt{pqr\_list} stores all the pairs of $(p,q)$ and $r$ we need}

        \item[]
        \STATE $\texttt{h\_diff\_list}\gets\texttt{[]}$
        \STATE
        \FOR{\texttt{var} \textbf{in} $h$:}%\COMMENT{\texttt{var} loops through all the variables (channels) of $h$}
        \STATE
        \STATE $\texttt{var\_diff\_list}\gets\texttt{[]}$
        \STATE
        \FOR{$(p,q), r$ \textbf{in} $\texttt{pqr\_list}$:}
        \STATE
        \STATE \texttt{Cuv} $\gets$ CNN{$h$, $p+q+r$}%\COMMENT{the parameters of CNNs vary according}
        \STATE \COMMENT{to different \texttt{var} and $((p,q), r)$}
        \FOR{\texttt{i,j} \textbf{in} grid point locations:}
        \STATE
        \STATE $(c_{uv})_{u+v>p+q+r}\gets\texttt{Cuv[i,j]}$%\COMMENT{aliasing}
        \STATE $\texttt{K[i,j]}\gets K_{pq}^0+\sum_{u+v>p+q+r}c_{uv}K_{uv}^0$%\COMMENT{by Prop. \ref{prop:kernels-in-hyperplane}}
        \STATE
        \ENDFOR
        \STATE
        \STATE $\texttt{conv[i,j]}\gets\sum_{\texttt{s,t}=-L}^L\texttt{K[i,j][s,t] * var[i+s,j+t]}$%\COMMENT{dynamic conv.}
        \STATE \textbf{append} \texttt{conv} \textbf{to} \texttt{var\_diff\_list}
        \STATE
        \ENDFOR
        %\Statex
        \STATE \textbf{append} \texttt{var\_diff\_list} \textbf{to} \texttt{h\_diff\_list}
        \STATE
        \ENDFOR
        \STATE \textbf{return} \texttt{h\_diff\_list}
        \STATE
        \ENDFUNCTION
        \STATE
        \FUNCTION{CNN($h$, $m$)}

        \STATE
        \STATE $\texttt{x}\gets\texttt{Relu}(\texttt{Conv2d}(h))$%\COMMENT{16 output channels}
        \STATE $\texttt{x}\gets\texttt{Relu}(\texttt{Conv2d}(\texttt{x}))$%\COMMENT{16 output channels}
        \STATE $\texttt{x}\gets\texttt{Conv2d}(\texttt{x})$%\COMMENT{$((2L+1)^2-\frac12m(m+1))$ output channels by Eq. (\ref{eq:channel-num})}
        \STATE \textbf{return} \texttt{x}
        \STATE
        \ENDFUNCTION
    \end{algorithmic}
\end{algorithm}

==> sections/fig_FN_snapshots.tex <==
\begin{figure}
    \begin{center}
        \centerline{\includegraphics[width=1.0\columnwidth]{./figs/exp_fn_result.pdf}}
        \caption{\textbf{RD equations:} Predicted snapshots at different time steps. `reference' represents ground truth; `Ours' indicates the prediction of PDE-Net++ (TDDL, FNO).
        }
        \label{fig:fn_result}
    \end{center}
\end{figure}

==> sections/fig_burgers_ablation.tex <==
\begin{figure}
    \begin{center}
        \centerline{\includegraphics[width=0.8\columnwidth]{./figs/exp_burgers_ablation_train_size.pdf}}
        \caption{\textbf{Burgers' equation:} Comparison of different methods under different numbers of training samples.}
        \label{fig:burgers_ablation_train_size}
    \end{center}
\end{figure}

==> sections/tab_NS_l2error.tex <==
\begin{table}
    \renewcommand{\arraystretch}{1.2} % 控制行距
    \centering
    \caption{\textbf{Navier-Stokes equation:} Comparison of different methods under different backbones.}
    \label{tb:ns_different_method}
    {\small
        \setlength{\tabcolsep}{1.5mm}{ % 控制单元格宽度
            \begin{tabular}{c | c | c | c  c}
                \hline
                \textbf{Backbone} & \textbf{Method} & \textbf{Derivatives} & \textbf{\textit{SR}}                 & \boldmath{$L_2$} \textbf{\textit{error}}                            \\
                \hline
                \multirow{5}{*}{U-Net}             & Black-Box                        & -                                     & 100\%                                & 5.276e-3         \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 98\%                                 & 8.029e-3         \\
                                                   &                                  & Moment                                & 100\%                                & 6.865e-3         \\
                                                   &                                  & Upwind                                & 100\%                                & 7.153e-3         \\
                                                   &                                  & TDDL                                  & 100\%                                & 2.748e-3         \\
                \hline
                \multirow{5}{*}{ConvResNet}        & Black-Box                        & -                                     & 100\%                                & 1.114e-1         \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 61\%                                 & 1.915e-3         \\
                                                   &                                  & Moment                                & 100\%                                & 1.819e-3         \\
                                                   &                                  & Upwind                                & 100\%                                & 1.936e-3         \\
                                                   &                                  & TDDL                                  & 100\%                                & 1.951e-3         \\
                \hline
                \multirow{5}{*}{FNO}               & Black-Box                        & -                                     & 100\%                                & 3.204e-3         \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 36\%                                 & 4.710e-3         \\
                                                   &                                  & Moment                                & 100\%                                & 7.471e-4         \\
                                                   &                                  & Upwind                                & 100\%                                & 7.971e-4         \\
                                                   &                                  & TDDL                                  & 100\%                                & 9.081e-4         \\
                \hline
                \multirow{5}{*}{F-FNO}             & Black-Box                        & -                                     & 100\%                                & 2.721e-3         \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 23\%                                 & 3.331e-3         \\
                                                   &                                  & Moment                                & 100\%                                & 1.265e-3         \\
                                                   &                                  & Upwind                                & 100\%                                & 1.291e-3         \\
                                                   &                                  & TDDL                                  & 100\%                                & 1.333e-3         \\
                \hline
                \multirow{5}{*}{\makecell[c]{Galerkin \\ Transformer}} & Black-Box    & -                                     & 100\%                                & 2.821e-2         \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 94\%                                 & 1.802e-3         \\
                                                   &                                  & Moment                                & 99\%                                 & 7.173e-3         \\
                                                   &                                  & Upwind                                & 100\%                                & 8.872e-3         \\
                                                   &                                  & TDDL                                  & 100\%                                & 1.041e-2         \\
                \hline
            \end{tabular}
        }
    }
\end{table}

==> sections/tab_burgers_l2error.tex <==
\begin{table}
    \renewcommand{\arraystretch}{1.2} % 控制行距
    \centering
    \caption{\textbf{Burgers' equation:} Comparison of different methods under different backbones.}
    \label{tb:burgers_different_method}
    {\small
        \setlength{\tabcolsep}{1.5mm}{ % 控制单元格宽度
            \begin{tabular}{c | c | c | c  c}
                \hline
                \textbf{Backbone} & \textbf{Method} & \textbf{Derivatives} & \textbf{\textit{SR}}                 & \boldmath{$L_2$} \textbf{\textit{error}}                                            \\
                \hline
                \multirow{5}{*}{U-Net}             & Black-Box                        & -                                     & 100\%                                & 9.718e-2                                 \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 96\%                                 & 7.624e-3                                 \\
                                                   &                                  & Moment                                & 100\%                                & 4.210e-3                                 \\
                                                   &                                  & Upwind                                & 100\%                                & 4.970e-3                                 \\
                                                   &                                  & TDDL                                  & 100\%                                & 3.114e-3                                 \\
                \hline
                \multirow{5}{*}{ConvResNet}        & Black-Box                        & -                                     & 100\%                                & 1.050e-1                                 \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 96\%                                 & 1.204e-2                                 \\
                                                   &                                  & Moment                                & 97\%                                 & 6.151e-3                                 \\
                                                   &                                  & Upwind                                & 100\%                                & 7.767e-3                                 \\
                                                   &                                  & TDDL                                  & 100\%                                & 4.481e-3                                 \\
                \hline
                \multirow{5}{*}{FNO}               & Black-Box                        & -                                     & 100\%                                & 1.162e-2                                 \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 98\%                                 & 1.036e-2                                 \\
                                                   &                                  & Moment                                & 99\%                                 & 4.345e-3                                 \\
                                                   &                                  & Upwind                                & 100\%                                & 4.664e-3                                 \\
                                                   &                                  & TDDL                                  & 100\%                                & 3.034e-3                                 \\
                \hline
                \multirow{5}{*}{F-FNO}             & Black-Box                        & -                                     & 100\%                                & 2.064e-2                                 \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 96\%                                 & 9.545e-3                                 \\
                                                   &                                  & Moment                                & 100\%                                & 4.529e-3                                 \\
                                                   &                                  & Upwind                                & 100\%                                & 4.456e-3                                 \\
                                                   &                                  & TDDL                                  & 100\%                                & 2.920e-3                                 \\
                \hline
                \multirow{5}{*}{\makecell[c]{Galerkin                                                                                                                                                           \\ Transformer}} & Black-Box & - & 100\% & 8.919e-2 \\
                \cline{2-5}
                                                   & \multirow{4}{*}{PDE-Net++}       & FDM                                   & 96\%                                 & 9.316e-3                                 \\
                                                   &                                  & Moment                                & 100\%                                & 5.473e-3                                 \\
                                                   &                                  & Upwind                                & 100\%                                & 5.307e-3                                 \\
                                                   &                                  & TDDL                                  & 100\%                                & 5.755e-3                                 \\
                \hline
            \end{tabular}
        }
    }
\end{table}
